CrossFit: A Few-shot Learning Challenge for Cross-task Generalization in NLP

Humans can learn a new language task efficiently with only few examples, by leveraging their knowledge obtained when learning prior tasks. In this paper, we explore whether and how such cross-task generalization ability can be acquired, and further applied to build better few-shot learners across diverse NLP tasks. We introduce CrossFit, a problem setup for studying cross-task generalization ability, which standardizes seen/unseen task partitions, data access during different learning stages, and the evaluation protocols. To instantiate different seen/unseen task partitions in CrossFit and facilitate in-depth analysis, we present the NLP Few-shot Gym, a repository of 160 diverse few-shot NLP tasks created from open-access NLP datasets and converted to a unified text-to-text format. Our analysis reveals that the few-shot learning ability on unseen tasks can be improved via an upstream learning stage using a set of seen tasks. We also observe that the selection of upstream learning tasks can significantly influence few-shot performance on unseen tasks, asking further analysis on task similarity and transferability.

==> figure_code/non-mcqa.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.98\textwidth]{figure/non-mcqa.pdf}
    % \vspace{-0.3cm}
    \caption{x}
    \label{fig:non-mcqa}
\end{figure*}

==> figure_code/non-mrc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figure/non-mrc.pdf}
    % \vspace{-0.3cm}
    \caption{x}
    \label{fig:non-mrc}
\end{figure}

==> figure_code/non-nli.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figure/non-nli.pdf}
    % \vspace{-0.3cm}
    \caption{x}
    \label{fig:non-nli}
\end{figure}

==> figure_code/non-paraphrase.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figure/non-paraphrase.pdf}
    % \vspace{-0.3cm}
    \caption{x}
    \label{fig:non-paraphrase}
\end{figure}

==> figure_code/random-test.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figure/random-test.pdf}
    \vspace{-0.3cm}
    \caption{Relative Performance Gain on $\mathcal{T}_{test}$ (Random split)}
    \label{fig:random-test}
\end{figure*}
